Choreographic Programming of Isolated Transactions

Implementing distributed systems is hard; choreographic programming aims to make it easier. In this paper, we present the design of a new choreographic programming language that supports isolated transactions among overlapping sets of processes. The first idea is to track for every variable which processes are permitted to use it. The second idea is to use model checking to prove isolation.

==> eptcsdata.tex <==
\providecommand{\firstpage}{49}
\providecommand{\publicationstatus}{Ilaria Castellani and Alceste Scalas (Ed.): 14th Workshop\\
on Programming Language Approaches to Concurrency and\\ Communication-cEntric Software (PLACES 2023).\\
EPTCS 378, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.378.5}{10.4204/EPTCS.378.5}}

